PyVision-RL: Forging Open Agentic Vision Models via RL

Reinforcement learning for agentic multimodal models often suffers from interaction collapse, where models learn to reduce tool usage and multi-turn reasoning, limiting the benefits of agentic behavior. We introduce PyVision-RL, a reinforcement learning framework for open-weight multimodal models that stabilizes training and sustains interaction. Our approach combines an oversampling-filtering-ranking rollout strategy with an accumulative tool reward to prevent collapse and encourage multi-turn tool use. Using a unified training pipeline, we develop PyVision-Image and PyVision-Video for image and video understanding. For video reasoning, PyVision-Video employs on-demand context construction, selectively sampling task-relevant frames during reasoning to significantly reduce visual token usage. Experiments show strong performance and improved efficiency, demonstrating that sustained interaction and on-demand visual processing are critical for scalable multimodal agents.

==> sections/1_introduction.tex <==
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{PyVision (arxiv)/figures/model_performance_comparison_broken_axis.png}
%     \caption{Our \model\ method with dynamic tool generation enables precise image modification, improving performance on various visual question answering benchmarks.}
%     \label{fig:pdf}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{ICLR 2025 Template/figures/grouped_comparison.pdf}
    \caption{\model\ improves performance on versatile VQA benchmarks compared to vanilla MLLMs.}
    \label{fig:pdf}
\end{figure}

\section{Introduction}
\vspace{5pt}
\label{sec:intro}

% Reviewing the development of multi-modal large language models (MLLM), this field has evolved from System 1-style multimodal models to those equipped with advanced long-chain reasoning capabilities. Recently, there has been a surge of research on integrating tool-use capabilities into MLLMs. By leveraging tool invocation such as cropping or rotating images, these models can enhance their understanding and reasoning over visual content.
% Broadly, existing works on MLLMs with tool-use can be categorized into two groups.

% \noindent
% \textbf{MLLM with Static Tool Set.}
% This category defines a fixed set of tools that the model can call. After appropriate training, the model can leverage these predefined tools during inference to assist its perception or reasoning. Representative works in this direction include DeepEyes, HuggingGPT, and MCP. By predefining domain-specific tools and carefully fine-tuning with tool-using trajectories, models can actively invoke tools during inference. %tuning their execution environments, these approaches ensure that models can reliably and actively invoke tools during inference. 

% \noindent
% Furthermore, when employing reinforcement learning to improve tool usage, the clear specification of tool functionalities and parameter formats within the model’s context makes it easier to assign rewards based on the rollouts. However, the reliance on a fixed toolset may also limit the model’s generalization and flexibility to new domains.

% \noindent
% \textbf{MLLM with Dynamic Tool Generation.}
% The second category focuses on dynamic tool generation, empowering models with the capability to write code and thereby generate and execute custom tools on-the-fly during inference. Notable examples in this direction include OpenAI’s o3 and o4-mini. Compared to the fixed toolset approach, dynamic tool generation enables models to autonomously create a wide variety of tools tailored to specific tasks, significantly enhancing generalization and versatility.

A defining feature of human intelligence is the ability to dynamically generate and adapt tools to solve novel problems. Unlike animals—whose tool use is limited to static, instinctual patterns (\eg chimpanzees reusing sticks for termite fishing)—humans innovate adaptively: we create diverse tools adapted to dynamic problems, enabling open-ended technological evolution.

\noindent
In AI, however, most agent systems still operate with a static toolset~\citep{hugginggpt,IEP,mmreact,visprog,visualsketchpad,23viper}—a predefined collection of functions or APIs akin to an animal’s fixed behavioral repertoire. While effective for narrow tasks, such rigidity limits adaptability; agents fail when faced with problems requiring unseen tool combinations or modifications.

\noindent
In this work, we propose \model, visual understanding with dynamic tool generation, as a paradigm shift. Inspired by human ingenuity, we equip agents with only a minimal primitive—a Python execution environment—and task them with autonomously generating, testing, and refining tools as code to address diverse challenges. Table.~\ref{tab:comp_visual_prog} shows the comparison between \model\ to other visual programming~\footnote{Visual programming refers to equipping LLM or MLLM with tools, \eg image process function or vision specialist. The LLM or MLLM solves visual tasks by compositional tool using.} methods. 


%Inspired by o3 and o4-mini, 
% While o3 and o4-mini achieves promising results recently, their closed-source nature limits transparency and reproducibility, prompting us to reproduce their approach. We begin exploration by asking whether current state-of-the-art MLLMs can be prompted to invoke their tool-using capabilities.
\noindent
We leverage MLLM (GPT-4.1~\citep{gpt4.1} and Claude-4.0-Sonnet~\citep{claude4}) to develop an image understanding agent capable of dynamically generating tools. Specifically, we construct a sophisticated system prompt that encourages MLLM to generate Python code and execute on the fly, provided with a Python execution environment equipped with essential image processing packages. The execution results of the generated code blocks—be they textual outputs or images—are captured by redirecting the standard output stream and extracting runtime variables, respectively. We concatenate these results back into MLLM dialogue history, enabling the model to iteratively write and refine code blocks over multiple turns, thereby progressively constructing comprehensive solutions to visual problems.

\noindent
We evaluate this system across a diverse set of visual domains, including mathematics, medical, remote sensing, visual puzzles, and chart. Remarkably, the agent is able to generate creative and sometimes unexpected tools tailored to each specific task. For instance, in medical question answering, the agent enhances and crops regions relevant to a disease; and for geometry problems, it renders auxiliary lines directly onto images as needed. We also conduct systematic evaluations on several benchmarks and observe consistent improvements over vanilla MLLM. Our core contributions are listed as follows:
\begin{itemize}
\item We propose \model, a novel approach where MLLMs, \eg GPT-4.1 and Claude-4.0-Sonnet, dynamically generate, test, and refine tools (as code) in a Python environment to solve diverse visual tasks, moving beyond static, predefined tool sets.
\item \model\ was evaluated on versatile benchmarks covering diverse domains. And has been proven effective in bringing performance improvement generally: +31.1\% on VLMsareBlind-mini~\citep{vlmsareblind}~\footnote{Since VLMsareBlind has 8k test samples, considering the limit of API budget, we uniformly sampled one-eighth of the data from each subtask to form VLMsareBlind-mini.}; +8.3\% on VisualPuzzles~\citep{song2025visualpuzzles}; +7.8\% on V* bench~\citep{wu2024vstar}.
\item We analyzed and categorized the pattern distribution of the dynamically generated tools in different benchmarks and domains. We found that when faced with problems from different domains, the model often tends to generate certain tools: for visual search task, model tends to generate crop-related tools; for medical task, model tends to generate enhancing contrast-related tools; for remote sensing tasks, model tends to generate segmentation-related tools.
\end{itemize}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=1\textwidth]{ICLR 2025 Template/figures/teaser-case-2.pdf}
    % \caption{The case shows \model's capability to accurately generating masks for center circles and calculating pixel counts — showing distinct behavior compared to MLLMs.}
    \caption{This is a question disguised as a Ebbinghaus illusion~\citep{jaeger2015ebbinghaus}, asking which of the two central balls is larger. We found that this image, with a pattern similar to that of the Ebbinghaus illusion problem, triggers hallucinations in MLLMs~\citep{gpt4.1}, causing it to mistakenly think this is a typical Ebbinghaus illusion question and then easily provide the wrong answer. However, for \model, it first calculates the colors of the two central balls, then creates a binary image that only retains the two central balls by filtering pixel values, and finally gives the correct answer: the ball on the right is larger.}
    \label{fig:pdf}
\end{figure}


\begin{table}[tbp]
    \centering
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{l|cccc}
    \toprule
    Methods& Predefined Workflow & Static Toolset & Execution on the Fly & Visual Parser~\citep{visualparser}\\
    \midrule
    NMN~\citep{neuralmodulenetwork} & \checkmark &  \checkmark &\texttimes & \checkmark \\
    IEP~\citep{IEP} & \checkmark &  \checkmark &\texttimes & \checkmark \\
     VisProg~\citep{visprog} & \texttimes & \checkmark &\texttimes & \checkmark\\
     Visual ChatGPT~\citep{visualchat} & \checkmark& \checkmark & \checkmark & \checkmark \\
     ViperGPT~\citep{23viper} & \texttimes& \checkmark & \texttimes& \checkmark\\
     MM-REACT~\citep{mmreact} & \checkmark & \checkmark &\texttimes & \checkmark\\
     HuggingGPT~\citep{hugginggpt} & \checkmark & \checkmark & \texttimes & \checkmark \\
     Image-of-Thought~\citep{iot} & \checkmark & \checkmark & \texttimes & \checkmark \\
     Visual Sketchpad~\citep{visualsketchpad} & \texttimes& \checkmark & \checkmark & \checkmark\\
     VAT~\citep{vat} & \checkmark & \checkmark & \texttimes& \checkmark\\
     \midrule
     \model\ (Ours) & \texttimes& \texttimes&\checkmark & \texttimes \\
     \bottomrule
    \end{tabular}}
    % \caption{Comparison to other visual programming methods.}
    \caption{Comparison to other visual programming methods. Predefined Workflow: }
    \label{tab:comp_visual_prog}
\end{table}


==> sections/3_method.tex <==
\section{PyVision}
\vspace{-5pt}
\label{sec:pyvision}

% \begin{figure}[bp]
%     \centering
%     \includegraphics[width=1\textwidth]{ICLR 2025 Template/figures/method.drawio-3.pdf}
%     \caption{\model\ pipeline for visual question answering. Instead of a single-step response, the system iteratively generates code, executes it, and incorporates the results back into the context. This process repeats until the model complete its generation, enabling multi-step reasoning.}
%     \label{fig:methos}
% \end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=1\textwidth]{PyVision (arxiv)/figures/method-zst.drawio-3.pdf}
    \caption{\model, an interactive and multi-turn framework capable of dynamic tool generation, designed for multi-modal reasoning. In an inference session, \model\ has $n$ interaction turns with the Python interpreter. $code\_block\_i$ and $mm\_clue\_i$ refer to the generated code by the MLLM and the executed output by the Python interpreter in the $i_{th}$ turn, $i=0,1,...,n$.}
    \label{fig:methods}
\end{figure}

We propose \model, an interactive, multi-turn framework for multimodal reasoning. Unlike previous works that rely on a predefined static toolset consisting of image processing operations and deep nets such as detection~\citep{groundingdino} and segmentation~\citep{kirillov2023sam} models, \model\ provides only a Python interpreter as a flexible tooling interface. Thanks to Python’s rich ecosystem and the strong coding capabilities of modern LLMs, we find that \model\ allows the generation of complex, adaptive tools tailored to a wide range of tasks and scenarios.

\subsection{Python as Tooling Backend}
The prerequisite for dynamic tooling is a flexible backend. In \model, we adopt Python as the building blocks of dynamic tooling. In this section, we first discuss the motivation behind choosing Python as our interface language and introduce how to implement the isolation between the environment and the main process. We then present two key features of the Python-based interface in \model.

% \paragraph{Simplicity.} 
% % If you want to deploy a deep learning model as an external tool in the inference environment, you need to first deploy the model on a GPU machine or a container with GPU resources and then wrap this model using FastAPI~\citep{lubanovic2023fastapi} or other API wrappers. During the inference process, the GPU machine must not be interrupted and must maintain good communication with the host. 
% Enabling Python as the interface, we do not need another machine or container, since Python inherently supports creating a Python runtime and executing a specific piece of code. It means we could implement the environment interaction within our code. But for better isolation, you could also use another container, \eg SandboxFusion~\citep{sandboxfusion} and E2B sandbox, with CPU resources to run the generated Python code.

\paragraph{Python's Rich Ecosystem.} Python offers an unparalleled collection of mature libraries for image and video processing (OpenCV~\citep{opencv}, Pillow~\citep{pillow}), numerical computation (NumPy~\citep{numpy}), data handling (Pandas~\citep{pandas}), scientific computation (SciPy~\citep{scipy}), machine learning (Scikit-learn~\citep{scilearn}, Scikit-image~\citep{sciimage}), \textit{etc}. These libraries provide a fertile ground for generating advanced tools.

\paragraph{Process-Level Isolation via Subprocess.} 
% If you want to deploy a deep learning model as an external tool in the inference environment, you need to first deploy the model on a GPU machine or a container with GPU resources and then wrap this model using FastAPI~\citep{lubanovic2023fastapi} or other API wrappers. During the inference process, the GPU machine must not be interrupted and must maintain good communication with the host. 
% Enabling Python as the interface, we do not need another machine or container, since Python inherently supports creating a Python runtime and executing a specific piece of code. It means we could implement the environment interaction within our code. But for better isolation, you could also use another container, \eg SandboxFusion~\citep{sandboxfusion} and E2B sandbox, with CPU resources to run the generated Python code.

After an MLLM generates Python code, this code must be executed by an additional Python runtime, which we refer to as the \textbf{runtime environment}. The isolation between the runtime environment and the main process runtime is crucial. Insufficient isolation may result in several undesirable consequences: (1) the environment runtime could modify variables in the main process; (2) it could corrupt the file system of the main process or even the host system; and (3) it may consume excessive host resources, potentially leading to termination of the main process.

To ensure necessary isolation, there are three feasible approaches to implementing the environment runtime: (1) dynamically spawning a subprocess within the main process to serve as the environment runtime~\citep{feng2025retool}, which provides isolation at the memory level~\footnote{Memory level isolation is the same as process level isolation, and we switch between these two terms.}; (2) leveraging a Jupyter kernel as the environment runtime~\citep{visualsketchpad}, which also only offers memory-level isolation; and (3) deploying Docker-based execution~\citep{sandboxfusion}, which achieves system-level isolation.

In \model, for reasons of ease of integration, we adopt the first approach: the main process dynamically spawns a subprocess as the environment runtime to execute the generated Python code. This strategy achieves process-level isolation between the environment runtime and the main process, while obviating the need for additional hosts or virtual machines.

\paragraph{Cross-Turn Persistent Environment.}
During a single inference session, \model\ engages in multiple rounds of interaction with the environment runtime, shown as in Fig.~\ref{fig:methods}. In the $i_{th}$ round, where $i=1,2,\dots,n$, the generated code may access variables from previous execution turns. Therefore, we need a runtime with cross-turn persistence.

In \model, we initialize a Python runtime at the beginning of each inference session and execute all subsequent interactions within this persistent environment. This design allows intermediate variables in different turns to be shared seamlessly across the session, thereby significantly enhancing the flexibility and capability of \model.

\paragraph{File System-Isolated I/O.}
In addressing the VQA task, \model\ frequently applies various image processing operations, such as cropping or visualizing specific image statistics. These newly generated visual cues need to be incorporated into the MLLM's context. Consequently, there exists a necessary I/O between the environment runtime and the MLLM context. There are two designs for implementing it: (1) utilizing the main process’s file system as an intermediary to facilitate I/O between the environment runtime and the MLLM context~\citep{thinkwithimage}, or (2) leveraging specific variables within the environment runtime to enable restricted variable-passing between the environment runtime and the MLLM context~\citep{feng2025retool}. Concretely, the latter approach involves the main process reading specific variables from the environment runtime to acquire intermediate results, which are then processed and incorporated into the MLLM context. In \model, we adopt the latter strategy. This approach eliminates direct interaction with the main process’ file system, offering improved isolation, security, and stability. In particular, for \textbf{MLLM context -> environment runtime}, we load the $i_{th}$ image in the MLLM's context using \lstinline{"PIL.Image.open()"} in the main process and inject into the variable \lstinline{"image_clue_i"} in the cross-turn persistent environment runtime. For \textbf{environment runtime -> MLLM context}, we inform the MLLM to use \lstinline{"plt.show()"} and \lstinline{"print()"} to output the intermediate results, and we redirect the corresponding variables, process and append them to the MLLM context.

\subsection{Visual Understanding with Dynamic Tool Generation}
% We propose a novel framework, \model, wherein the MLLM is provided with a Python interpreter as the primitive tool. The model can then generate and execute code to perform various operations on the input image, such as cropping or rotating. The resulting outputs are subsequently fed back into the model's context, creating a multi-turn interaction with the Python environment that aids the model's multi-modal reasoning. To realize this objective, we introduce two core designs as follows:
In this section, we detail how dynamic tool creation is achieved by designing system prompts for MLLMs. Furthermore, we analyze the differences between dynamic tool generation and traditional tool using methods.

\noindent
\textbf{System Prompt.} 
Since \model\ is a training-free framework, we designed a comprehensive system prompt to teach the model output as our desired structure.

\begin{tcolorbox}[
    title={A Glimpse of the System Prompt},
    colback=blue!5!white,
    colframe=blue!40!white,
    left=1mm, right=1mm, top=1mm, bottom=1mm,
    width=\textwidth,
    center,
    fonttitle=\small,
    fontupper=\small,
    label=prompt_snake_agent
]
{
\dots \\
\\
For all the provided images, in order, the i-th image has already been read into the global variable \lstinline{"image_clue_i"} using the \lstinline{"PIL.Image.open()"} function. When writing Python code, you can directly use these variables without needing to read them again. \\
\dots \\
\\
Note that when you use matplotlib to visualize data or further process images, you need to use \lstinline{"plt.show()"} to display these images; there is no need to save them. Do not use image processing libraries like cv2 or PIL. If you want to check the value of a variable, you MUST use \lstinline{"print()"} to check it. \\
\dots \\
\\
Each code snippet is wrapped with <code> \\
'''python \\
code snippet \\
``` \\
</code>. \\
\dots \\
\\
The last part of your response should be in the following format: \\
<answer>\lstinline|\boxed{"The final answer goes here."}|</answer> \\
\dots

}
\end{tcolorbox}

% By restricting the output's structure, we could parse the generated Python code and execute it during inference time. By restricting the final answer's output format, we could parse the answer and evaluate it conveniently. 

\noindent
In the system prompt, we inform the MLLM that the $i_{th}$ image in the context has already been sequentially loaded into the environment runtime as the variable \lstinline{"image_clue_i"} using \lstinline{"PIL.Image.open()"}, allowing for direct access and manipulation. Additionally, we instruct the MLLM to utilize \lstinline{"plt.show()"} and \lstinline{"print()"} for outputting visual and textual variables that are helpful for reasoning. This approach explicitly tells the I/O protocol between the MLLM context and the environment runtime, enabling the MLLM to generate Python code that adheres to our designed file system-isolated I/O conventions. Moreover, we specify the expected formats for both the generated Python code and the final answer within the system prompt, facilitating the subsequent parsing of code and answers.
The full system prompt is in Appendix Sec.~\ref{sec:prompt_appendix}.

\noindent
\textbf{Dynamic Tool Generation.} 
% The foundation of enabling MLLM to interact with the multi-modal input lies in "tool calling", where an MLLM can call a predefined tool with specified arguments. Traditionally, developers define these tools in advance, including their expected inputs and outputs~\citep{23viper,hugginggpt,visprog,visualsketchpad}. However, \model\ introduces a more adaptable and flexible approach—leveraging MLLM to dynamically generate tools and execute them on the fly.
By integrating the three components described above—\textbf{cross-turn persistent runtime}, \textbf{file system-isolated I/O}, and \textbf{system prompt}—we implement \model. As illustrated in Fig.~\ref{fig:methods}, during an inference session, the system prompt and image-question pair are provided as input to the MLLM. The MLLM then performs reasoning and generates adaptive Python code, termed as $code\_block\_0$, to further process the input. The generated code is executed in the cross-turn persistent runtime, producing execution results that include both textual and visual content, termed as $mm\_clue\_0$. $mm\_clue\_0$ are subsequently fed back into the MLLM's context. This interaction is repeated for $n+1$ turns, after which the MLLM integrates the initial input and the multi-modal rationale to produce the final answer.

PyVision distinguishes itself from previous works in four key aspects during the inference process as in Table.~\ref{tab:comp_visual_prog}:
(1) No Fixed Workflow: Unlike approaches such as HuggingGPT~\citep{hugginggpt}, \model\ does not follow a predefined workflow. The MLLM autonomously decides the number of interactions with the environment and when to terminate the session to provide the final answer.
(2) No Fixed Toolset: In contrast to works like Visual Sketchpad~\citep{visualsketchpad}, \model\ allows the MLLM to dynamically create a wide variety of tools for image or text processing via Python code, rather than relying on a fixed set of tools.
(3) Multi-turn Interaction: \model\ operates as a multi-turn interaction process, setting it apart from methods such as VisProg~\citep{visprog} and HuggingGPT~\citep{hugginggpt}, which are typically single-turn or less adaptive.
(4) No Dependence on External Visual Neural Networks: \model\ achieves comprehensive image processing solely through the MLLM and Python code, without requiring other visual neural networks (NNs), which further differentiates it from systems like Visual Sketchpad~\citep{visualsketchpad}.

% A dynamically generated tool~\citep{dynamictool} refers to a function or code snippet created by the MLLM in real-time based on the multi-modal input and the previous multi-modal rationale. This eliminates the need to consider every possible scenario, allowing for more open-ended, creative, and adaptive problem-solving. We study and categorize the dynamically generated tools. And we find that (1) the MLLM creates some tools we never anticipated, \eg use the scikit-image~\citep{sciimage} package to implement image segmentation in a remote sensing task or draw an image histogram to count the specific patterns in an image. (2) The dynamically generated tools can be broadly categorized into four types: \textbf{basic image process}, \textbf{advanced image process}, \textbf{add visual prompts} and \textbf{mathematical and statistical analysis}.  More details are in Sec.~\ref{sec:case_study} and Sec.~\ref{sec:tool_taxonomy}.


\begin{table}[tbp]
    \centering
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{l|cccc}
    \toprule
    Methods& Predefined Workflow & Static Toolset & Multiple Turns & Other Visual NNs~\citep{visualparser} \\
    \midrule
    NMN~\citep{neuralmodulenetwork} & \checkmark &  \checkmark &\texttimes & \checkmark \\
    IEP~\citep{IEP} & \checkmark &  \checkmark &\texttimes & \checkmark \\
     VisProg~\citep{visprog} & \checkmark & \checkmark &\texttimes & \checkmark\\
     Visual ChatGPT~\citep{visualchat} & \checkmark& \checkmark & \checkmark & \checkmark \\
     ViperGPT~\citep{23viper} & \checkmark& \checkmark & \texttimes& \checkmark\\
     MM-REACT~\citep{mmreact} & \checkmark & \checkmark &\texttimes & \checkmark\\
     HuggingGPT~\citep{hugginggpt} & \checkmark & \checkmark & \texttimes & \checkmark \\
     Image-of-Thought~\citep{iot} & \checkmark & \checkmark & \texttimes & \checkmark \\
     Visual Sketchpad~\citep{visualsketchpad} & \texttimes& \checkmark & \checkmark & \checkmark\\
     VAT~\citep{vat} & \checkmark & \checkmark & \texttimes& \checkmark\\
     \midrule
     \model\ (Ours) & \texttimes& \texttimes&\checkmark & \texttimes \\
     \bottomrule
    \end{tabular}}
    % \caption{Comparison to other visual programming methods.}
    \caption{Comparison to other multi-modal tool using methods. }
    \label{tab:comp_visual_prog}
\end{table}




==> sections/6_discussion.tex <==
\vspace{-5pt}
\section{Discussion and Future Work}
\vspace{-8pt}
\label{sec:discussion}

\model\ is a training-free framework, implemented with only manually designed system prompts, frontier MLLM API~\citep{gpt4.1,claude4, team2023gemini} and a Python execution environment. Dynamic tool generation is the biggest feature and we saw the huge potential of it in solving diverse visual tasks. In the future, we plan to collect the rollout data generated by \model-gpt or \model-claude on diverse domains, explored in this paper. And fine-tune the open-source MLLMs~\citep{bai2025qwen25vl,team2025kimi,zhu2025internvl3} using these data with supervised fine-tuning and reinforcement learning to incentivise the dynamic tool generation ability of these models.



